Sequential Causal Discovery with Noisy Language Model Priors

Causal discovery from observational data typically assumes access to complete data and availability of perfect domain experts. In practice, data often arrive in batches, are subject to sampling bias, and expert knowledge is scarce. Language Models (LMs) offer a surrogate for expert knowledge but suffer from hallucinations, inconsistencies, and bias. We present a hybrid framework that bridges these gaps by adaptively integrating sequential batch data with LM-derived noisy, expert knowledge while accounting for both data-induced and LM-induced biases. We propose a representation shift from Directed Acyclic Graph (DAG) to Partial Ancestral Graph (PAG), that accommodates ambiguities within a coherent framework, allowing grounding the global LM knowledge in local observational data. To guide LM interactions, we use a sequential optimization scheme that adaptively queries the most informative edges. Across varied datasets and LMs, we outperform prior work in structural accuracy and extend to parameter estimation, showing robustness to LM noise.

==> tables/tbl_bg_noise_levels.tex <==
\begin{tabular}{|c|*{8}{c|}}
	\hline
	\multicolumn{9}{|c|}{Score}  \\
	\hline
	{$\rho$} & Batch 1 & Batch 2 & Batch 3 & Batch 4 & Batch 5 & Batch 6 & Batch 7& Total Interactions \\
	\hline
	$0.1$ & \val{8.7}{0.8} & \val{16.9}{0.8} & \val{17.2}{0.9} & \val{18.0}{0.9} & \val{18.4}{1.1} & \val{18.8}{1.1} & \val{19.0}{1.3} & \val{494.0}{162.37} \\
	$0.3$ & \val{3.9}{1.8} & \val{17.1}{0.8} & \val{18.6}{0.8} & \val{19.0}{0.9} & \val{19.4}{0.9} & \val{19.6}{0.9} & \val{19.8}{1.0} & \val{494.0}{113.33} \\
	$0.5$ & \val{0.8}{0.9} & \val{6.4}{1.9} & \val{10.9}{2.5} & \val{12.5}{1.8} & \val{13.4}{2.4} & \val{14.6}{2.2} & \val{15.5}{2.0} & \val{910.0}{0.0} \\
	$0.7$ & \val{0.1}{0.3} & \val{0.5}{0.7} & \val{1.1}{1.2} & \val{1.4}{1.2} & \val{1.4}{1.2} & \val{1.4}{1.2} & \val{1.5}{1.1} & \val{910.0}{0.0} \\
	$0.9$ & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{910.0}{0.0} \\
	\hline
	\multicolumn{9}{|c|}{Random} \\
	\hline
	{$\rho$} & Batch 1 & Batch 2 & Batch 3 & Batch 4 & Batch 5 & Batch 6 & Batch 7 & Total Interactions \\
	\hline
	$0.1$ & \val{4.3}{1.4} & \val{16.3}{0.8} & \val{17.6}{1.5} & \val{18.5}{1.5} & \val{18.7}{1.7} & \val{18.8}{1.7} & \val{19.1}{1.8} & \val{507.0}{122.64} \\
	$0.3$ & \val{1.9}{1.0} & \val{13.1}{1.0} & \val{16.7}{1.1} & \val{17.4}{1.4} & \val{18.0}{1.4} & \val{18.3}{1.5} & \val{18.6}{1.4} & \val{585.0}{104.81} \\
	$0.5$ & \val{0.3}{0.5} & \val{4.5}{1.3} & \val{6.4}{1.7} & \val{8.1}{1.9} & \val{9.2}{2.1} & \val{10.0}{2.2} & \val{11.3}{2.4} & \val{910.0}{0.0} \\
	$0.7$ & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.2}{0.4} & \val{0.2}{0.4} & \val{0.2}{0.4} & \val{0.2}{0.4} & \val{0.2}{0.4} & \val{910.0}{0.0} \\
	$0.9$ & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{0.0}{0.0} & \val{910.0}{0.0} \\
	\hline
\end{tabular}

==> tables/tbl_causal_discovery_metrics.tex <==
\begin{tabular}{cclccccc}
	\toprule
	\textbf{Dataset} & \textbf{Approach} & \textbf{Method} & \textbf{Mod. SHD $\downarrow$} & \textbf{SID $\downarrow$} & \textbf{Precision $\uparrow$} & \textbf{Recall $\uparrow$} & \textbf{F1 Score $\uparrow$} \\
	\midrule
\multirow{7}{*}{\rotatebox{90}{\dataset{Earthquake}{5}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{2.00}{0.00} & \val{(0.00, 5.00)}{(0.00, 0.00)} & \valb{1.00}{0.00} & \val{0.50}{0.00} & \val{0.67}{0.00} \\
&& FCI-Vanilla & \val{3.60}{0.80} & \val{(8.20, 9.20)}{(3.60, 1.60)} & \val{0.20}{0.40} & \val{0.05}{0.10} & \val{0.08}{0.16} \\
&& FCI-Iterative & \val{5.00}{1.67} & \val{(12.20, 12.20)}{(4.66, 4.66)} & \val{0.30}{0.27} & \val{0.20}{0.19} & \val{0.24}{0.22} \\
&& FCI-Heuristics & \val{3.60}{0.80} & \val{(8.20, 9.20)}{(3.60, 1.60)} & \val{0.20}{0.40} & \val{0.05}{0.10} & \val{0.08}{0.16} \\
\cdashline{2-8}[.4pt/1pt]
& \multirow{3}{*}{Data-LM} & LLM-first & \val{6.00}{0.82} & \val{(15.00, 15.00)}{(0.82, 0.82)} & \val{0.11}{0.16} & \val{0.08}{0.12} & \val{0.09}{0.13} \\
&& ILS-CSL & \val{2.38}{0.96} & \val{(5.25, 6.50)}{(0.83, 2.69)} & \valb{0.88}{0.22} & \val{0.44}{0.21} & \val{0.56}{0.21} \\
\rowcolor{highlight}\cellcolor{white} &\cellcolor{white}& \ours & \valb{1.00}{0.63} & \valb{(2.20, 2.20)}{(1.60, 1.60)} & \valb{1.00}{0.00} & \valb{0.75}{0.16} & \valb{0.85}{0.11} \\
	\midrule
\multirow{7}{*}{\rotatebox{90}{\dataset{Asia}{8}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{7.00}{0.00} & \val{(23.00, 49.00)}{(0.00, 0.00)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
&& FCI-Vanilla & \val{7.80}{0.75} & \val{(30.00, 35.00)}{(5.90, 2.45)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
&& FCI-Iterative & \val{8.00}{1.26} & \val{(33.00, 33.00)}{(7.46, 7.46)} & \val{0.45}{0.24} & \val{0.23}{0.15} & \val{0.29}{0.18} \\
&& FCI-Heuristics & \val{7.80}{0.75} & \val{(30.00, 35.00)}{(5.90, 2.45)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
\cdashline{2-8}[.4pt/1pt]
& \multirow{3}{*}{Data-LM} & LLM-first & \val{7.33}{0.94} & \val{(27.67, 27.67)}{(2.49, 2.49)} & \val{0.58}{0.12} & \val{0.29}{0.06} & \val{0.39}{0.08} \\
&& ILS-CSL & \val{6.50}{0.50} & \val{(28.50, 28.50)}{(3.20, 3.20)} & \valb{0.79}{0.12} & \val{0.28}{0.11} & \val{0.40}{0.12} \\
\rowcolor{highlight}\cellcolor{white} &\cellcolor{white}& \ours & \valb{4.60}{1.02} & \valb{(13.60, 13.60)}{(3.83, 3.83)} & \valb{0.80}{0.12} & \valb{0.60}{0.12} & \valb{0.67}{0.08} \\
	\midrule
	\multirow{7}{*}{\rotatebox{90}{\tiny\dataset{User Level Data-I}{9}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{15.00}{2.77} & \val{(47.80, 47.80)}{(4.62, 4.62)} & \val{0.72}{0.18} & \val{0.37}{0.09} & \val{0.47}{0.09} \\
	&& FCI-Vanilla & \val{21.30}{3.50} & \val{(61.60, 61.60)}{(5.54, 5.54)} & \val{0.41}{0.18} & \val{0.22}{0.10} & \val{0.29}{0.13} \\
	&& FCI-Iterative & \valb{\phantom{0}5.60}{1.20} & \val{(23.40, 23.40)}{(7.94, 7.94)} & \valb{0.93}{0.04} & \val{0.77}{0.02} & \valb{0.84}{0.03} \\
	&& FCI-Heuristics & \val{21.30}{3.50} & \val{(61.60, 61.60)}{(5.54, 5.54)} & \val{0.41}{0.18} & \val{0.22}{0.10} & \val{0.29}{0.13} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM} & LLM-first & \val{\phantom{0}9.68}{1.67} & \val{(38.12, 38.12)}{(4.06, 4.06)} & \val{0.80}{0.06} & \val{0.66}{0.04} & \val{0.72}{0.05} \\
	&& ILS-CSL & \val{\phantom{0}9.20}{1.72} & \val{(34.20, 34.20)}{(3.49, 3.49)} & \val{0.82}{0.05} & \val{0.66}{0.05} & \val{0.73}{0.05} \\
	 &  & \cellcolor{highlight} \ours & \cellcolor{highlight} \valb{\phantom{0}5.00}{0.71} & \cellcolor{highlight} \valb{(13.75, 13.75)}{(2.49, 2.49)} & \cellcolor{highlight} \valb{0.90}{0.04} & \cellcolor{highlight} \valb{0.83}{0.02} & \cellcolor{highlight} \valb{0.86}{0.02} \\
	\midrule
\multirow{7}{*}{\rotatebox{90}{\tiny\dataset{User Level Data-II}{8}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{19.80}{2.04} & \valb{(40.00, 40.00)}{(3.03, 3.03)} & \val{0.15}{0.07} & \val{0.10}{0.04} & \val{0.12}{0.05} \\
&& FCI-Vanilla & \val{17.40}{1.83} & \valb{(36.80, 39.40)}{(2.04, 3.38)} & \val{0.07}{0.13} & \val{0.02}{0.03} & \val{0.03}{0.05} \\
&& FCI-Iterative & \val{20.60}{1.77} & \val{(42.80, 43.40)}{(4.07, 4.22)} & \val{0.06}{0.08} & \val{0.05}{0.07} & \val{0.05}{0.07} \\
&& FCI-Heuristics & \val{17.40}{1.83} & \valb{(36.80, 39.40)}{(2.04, 3.38)} & \val{0.07}{0.13} & \val{0.02}{0.03} & \val{0.03}{0.05} \\
\cdashline{2-8}[.4pt/1pt]
& \multirow{3}{*}{Data-LM} & LLM-first & \val{18.75}{0.43} & \val{(44.00, 44.00)}{(1.00, 1.00)} & \val{0.18}{0.01} & \valb{0.17}{0.00} & \valb{0.18}{0.00} \\
&& ILS-CSL & \valb{16.90}{1.50} & \val{(44.40, 47.80)}{(6.05, 3.49)} & \val{0.16}{0.03} & \val{0.10}{0.04} & \val{0.12}{0.03} \\
 & & \cellcolor{highlight} \ours & \cellcolor{highlight} \valb{16.33}{1.80} & \cellcolor{highlight} \valb{(40.17, 40.17)}{(3.14, 3.14)} & \cellcolor{highlight} \valb{0.26}{0.04} & \cellcolor{highlight} \valb{0.18}{0.06} & \cellcolor{highlight} \valb{0.20}{0.04} \\
 \midrule
\multirow{7}{*}{\rotatebox{90}{\dataset{Child}{19}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{27.50}{0.00} & \valb{(111.00, 131.00)}{(0.00, 0.00)} & \val{0.38}{0.00} & \val{0.36}{0.00} & \val{0.37}{0.00} \\
&& FCI-Vanilla & \val{28.00}{1.48} & \val{(129.20, 133.20)}{(10.46, 10.76)} & \val{0.38}{0.04} & \val{0.26}{0.05} & \val{0.31}{0.04} \\
&& FCI-Iterative & \val{32.10}{1.16} & \val{(149.00, 164.40)}{(7.16, 10.33)} & \val{0.27}{0.03} & \val{0.26}{0.04} & \val{0.26}{0.03} \\
&& FCI-Heuristics & \val{28.00}{1.48} & \val{(129.20, 133.20)}{(10.46, 10.76)} & \val{0.38}{0.04} & \val{0.26}{0.05} & \val{0.31}{0.04} \\
\cdashline{2-8}[.4pt/1pt]
& \multirow{3}{*}{Data - LLM} & LLM-first & \val{31.67}{2.05} & \val{(172.00, 172.00)}{(13.42, 13.42)} & \val{0.29}{0.05} & \val{0.30}{0.05} & \val{0.30}{0.05} \\
&& ILS-CSL  & \val{32.00}{2.10} & \val{(154.00, 154.00)}{(26.53, 26.53)} & \val{0.28}{0.05} & \val{0.28}{0.05} & \val{0.28}{0.05} \\
\rowcolor{highlight}\cellcolor{white} &\cellcolor{white}& \ours & \valb{25.50}{0.89} & \valb{(103.40, 112.20)}{(8.09, 7.05)} & \valb{0.43}{0.01} & \valb{0.44}{0.02} & \valb{0.43}{0.01} \\
\midrule
\multirow{7}{*}{\rotatebox{90}{\dataset{Alarm}{37}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \valb{45.00}{0.00} & \valb{(626.00, 626.00)}{(\phantom{0}0.00, \phantom{0}0.00)} & \val{0.25}{0.00} & \val{0.02}{0.00} & \val{0.04}{0.00} \\
&& FCI-Vanilla & \val{49.50}{1.61} & \val{(617.80, 699.20)}{(29.23, 68.43)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
&& FCI-Iterative & \val{52.40}{6.21} & \valb{(612.20, 636.80)}{(49.87, 43.83)} & \valb{0.33}{0.14} & \val{0.12}{0.05} & \val{0.17}{0.07} \\
&& FCI-Heuristics & \val{49.50}{1.61} & \val{(617.80, 699.20)}{(29.23, 68.43)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
\cdashline{2-8}[.4pt/1pt]
& \multirow{3}{*}{Data - LLM} & LLM-first & \val{52.33}{3.09} & \val{(673.33, 673.33)}{(25.63, 25.63)} & \valb{0.33}{0.08} & \val{0.13}{0.02} & \val{0.19}{0.03} \\
&& ILS-CSL  & \val{51.20}{1.60} & \val{(657.20, 657.20)}{(24.07, 24.07)} & \val{0.34}{0.05} & \val{0.10}{0.01} & \val{0.15}{0.02} \\
\rowcolor{highlight}\cellcolor{white} &\cellcolor{white}& \ours & \val{50.90}{1.32} & \valb{(589.80, 591.00)}{(26.48, 25.59)} & \valb{0.42}{0.03} & \valb{0.22}{0.02} & \valb{0.29}{0.02} \\
\bottomrule
\end{tabular}

==> tables/tbl_causal_discovery_metrics_all_temp.tex <==
\begin{tabular}{ccccccc}
	\toprule
	\textbf{Dataset}& \textbf{Approach} & \textbf{Method} & \textbf{Mod. SHD} & \textbf{SID} & \textbf{Precision} & \textbf{Recall}\\
	\midrule
	\multirow{13}{*}{Earthquake} & \multirow{4}{*}{Only-Data} & FCI-Cumulative &\val{2}{0}&\val{(0, 5)}{(0,0)}&\val{1}{0}&\val{0.5}{0} \\
	&& FCI-Vanilla &\val{4}{0}&\val{(10, 10)}{(0,0)}&\val{0}{0}&\val{0}{0}  \\
	&& FCI-Iterative &\val{4}{0}&\val{(10, 10)}{(0,0)}&\val{0}{0}&\val{0}{0} \\
	&& FCI-Heuristics &\val{4}{0}&\val{(10, 10)}{(0,0)}&\val{0}{0}&\val{0}{0} \\
	\cdashline{2-7}[.4pt/1pt]
	& \multirow{3}{*}{LLM-Data}& LLM-first (t=0) & \val{4}{0} & \val{(10, 10)}{(0, 0)} & \val{0}{0} & \val{0}{0}  \\
	&& LLM-first (t=0.5) &\val{4}{0} & \val{(10, 10)}{(0, 0)} & \val{0}{0} & \val{0}{0}  \\
	&& LLM-first (t=1) &\val{4}{0} & \val{(10, 10)}{(0, 0)} & \val{0}{0} & \val{0}{0} \\
	\cdashline{2-7}[.4pt/1pt]
	&\multirow{6}{*}{Data-LLM} & ILS-CSL\textsubscript{FCI} (t=0) & \val{4}{0} & \val{(10,10)}{(0,0)} & \val{0}{0} & \val{0}{0} \\
	&  & ILS-CSL\textsubscript{FCI}(t=0.5) &  \val{4}{0} & \val{(10,10)}{(0,0)} & \val{0}{0} & \val{0}{0} \\
	&& ILS-CSL\textsubscript{FCI} (t=1) &  \val{4}{0} & \val{(10,10)}{(0,0)} & \val{0}{0} & \val{0}{0} \\
	& & Ours (t=0) &\val{2}{0} & \val{(5, 5)}{(0, 0)} & \val{0.75}{0} & \val{0.75}{0} \\
	&& Ours (t=0.5) & \val{2}{0} & \val{(5, 5)}{(0, 0)} & \val{0.85}{0.12} & \val{0.85}{0.12}  \\
	&& Ours (t=1) &\val{1.4}{0.9} & \val{(3.5, 3.5)}{(2.3, 2.3)} & \val{0.85}{0.12} & \val{0.85}{0.12} \\
	\midrule
	\multirow{13}{*}{Asia} & \multirow{4}{*}{Only-Data} & FCI-Cumulative &\val{7}{0}&\val{(23, 49)}{(0,0)}&\val{0}{0}&\val{0}{0} \\
	&& FCI-Vanilla &\val{9}{0}&\val{(37, 37)}{(0,0)}&\val{0}{0}&\val{0}{0} \\
	&& FCI-Iterative &\val{12}{0}&\val{(53, 53)}{(0,0)}&\val{0}{0}&\val{0}{0} \\
	&& FCI-Heuristics &\val{11}{0}&\val{(52, 52)}{(0,0)}&\val{0}{0}&\val{0}{0} \\
	\cdashline{2-7}[.4pt/1pt]
	& \multirow{3}{*}{LLM-Data} & LLM-first (t=0) &\val{9.0}{0.0} & \val{(44, 44)}{(0, 0)} & \val{0.4}{0.0} & \val{0.25}{0.0} \\
	&& LLM-first (t=0.5) &\val{9.0}{0.0} & \val{(44, 44)}{(0, 0)} & \val{0.4}{0.00} & \val{0.25}{0.00} \\
	&& LLM-first (t=1) &\val{9.0}{0.0} & \val{(44, 44)}{(0, 0)} & \val{0.4}{0.0} & \val{0.25}{0.00} \\
	\cdashline{2-7}[.4pt/1pt]
	&\multirow{6}{*}{Data-LLM} & ILS-CSL\textsubscript{FCI} (t=0) & \val{9.0}{0.0} & \val{(37, 37)}{(0,0)} & \val{0}{0} & \val{0}{0} \\
	&  & ILS-CSL\textsubscript{FCI} (t=0.5) & \val{9.0}{0.0} & \val{(37, 37)}{(0,0)} & \val{0}{0} & \val{0}{0} \\
	&& ILS-CSL\textsubscript{FCI} (t=1) & \val{9.0}{0.0} & \val{(37, 37)}{(0,0)} & \val{0}{0} & \val{0}{0} \\
	& & Ours (t=0) &\val{5.0}{0.0} & \val{(17, 17)}{(0,0)} & \val{0.8}{0} & \val{0.5}{0}  \\
	&& Ours (t=0.5) &\val{5.0}{0.0} & \val{(17, 17)}{(0,0)} & \val{0.8}{0} & \val{0.5}{0} \\
	&& Ours (t=1) &\val{5.0}{0.0} & \val{(17, 17)}{(0,0)} & \val{0.8}{0} & \val{0.5}{0} \\
	\midrule
	\multirow{13}{*}{User Data}  & \multirow{4}{*}{Only-Data}& FCI-Cumulative &\val{18.5}{0}&\val{(47, 47)}{(0,0)}&\val{0.7}{0}&\val{0}{0.37} \\
	&& FCI-Vanilla &\val{21}{0}&\val{(51, 51)}{(0,0)}&\val{0.38}{0}&\val{0.16}{0} \\
	&& FCI-Iterative &\val{4}{0}&\val{(20, 20)}{(0,0)}&\val{0.94}{0}&\val{0.84}{0} \\
	&& FCI-Heuristics &\val{6.5}{0}&\val{(22, 35)}{(0,0)}&\val{0.93}{0}&\val{0.74}{0} \\
	\cdashline{2-7}[.4pt/1pt]
	& \multirow{3}{*}{LLM-Data} & LLM-first (t=0) &\val{7}{0}&\val{(35,35)}{(0,0)}&\val{0.87}{0}&\val{0.74}{0} \\
	&& LLM-first (t=0.5) &\val{9.2}{0.6}  &\val{(42.5, 42.5)}{(3.3, 3.3)}& \val{0.81}{0.02}& \val{0.68}{0.02} \\
	&& LLM-first (t=1) &\val{8.7}{1.55} &\val{(39.4, 39.4)}{(4.34, 4.34)}& \val{0.82}{0.05}&\val{0.69}{0.04} \\
	\cdashline{2-7}[.4pt/1pt]
	&\multirow{6}{*}{Data-LLM} & ILS-CSL\textsubscript{FCI} (t=0) & \val{17.7}{1.07} & \val{(59.1, 59.3)}{(0.3, 0.49)} & \val{0.55}{0.03} & \val{0.41}{0.02} \\
	&  & ILS-CSL\textsubscript{FCI} (t=0.5) & \val{16.8}{0.60} & \val{(58.8, 58.8)}{((0.6, 0.6)} & \val{0.58}{0.02} & \val{0.43}{0.02} \\
	&& ILS-CSL\textsubscript{FCI} (t=1) & \val{18.3}{1.86} & \val{(57.2, 59.1)}{(6.79, 2.81)} &\val{0.53}{0.05} & \val{0.39}{0.05} \\
	& & Ours (t=0) &\val{3.4}{0.66} & \val{(3.7, 3.7)}{(4.12, 4.12)} & \val{0.90}{0.01} &\val{0.92}{0.03} \\
	&& Ours (t=0.5) &\val{3.3}{1.18} &\val{(3.6, 4.7)}{(5.8,7.4)}&\val{0.91}{0.02}&\val{0.92}{0.05} \\
	&& Ours (t=1) &\val{3.6}{0.93} &\val{(6.7, 6.7)}{(5.44, 5.44)}&\val{0.91}{0.02}&\val{0.9}{0.04} \\
	\midrule
	\multirow{13}{*}{User Data - 2}  & \multirow{4}{*}{Only-Data}& FCI-Cumulative & \val{19.7}{1.47} & \val{(36.2, 36.2)}{(1.94, 1.94)}& \val{0.11}{0.14} & \val{0.07}{0.08} \\
	&& FCI-Vanilla &\val{21.1}{1.58}&\val{(37.3, 37.3)}{(3.20, 3.20)}& \val{0.10}{0.11}&\val{0.06}{0.07} \\
	&& FCI-Iterative &\val{22.85}{1.23}& \val{(41.2, 42.5)}{(1.94, 1.69)} & \val{0.04}{0.07}& \val{0.03}{0.05} \\
	&& FCI-Heuristics & \val{20.35}{1.57} & \val{(37.2, 38.0)}{(2.18, 3.19)} & \val{0.06}{0.10} & \val{0.04}{0.06} \\
	\cdashline{2-7}[.4pt/1pt]
	& \multirow{3}{*}{LLM-Data} & LLM-first (t=0) & \val{17.2}{1.03} & \val{(43.4, 43.4)}{(1.26, 1.26)} & \val{0.27}{0.05} & \val{0.26}{0.06} \\
	&& LLM-first (t=0.5) & \val{18.1}{0.94} & \val{(44.1, 44.1)}{(0.7, 0.7)} & \val{0.24}{0.04} & \val{0.23}{0.05}  \\
	&& LLM-first (t=1) & \val{18}{0.07} & \val{(44.6, 44.6)}{(2.29, 2.29)} & \val{0.24}{0.03} & \val{0.23}{0.03}  \\
	\cdashline{2-7}[.4pt/1pt]
	&\multirow{6}{*}{Data-LLM} & ILS-CSL\textsubscript{FCI} (t=0) & \val{12.9}{1.39} & \val{(40, 40.9)}{(5.06, 5.24)} & \val{0.29}{0.21} & \val{0.19}{0.16} \\
	&  & ILS-CSL\textsubscript{FCI} (t=0.5) & \val{13.05}{1.78} & \val{(39.5, 39.5)}{(5.14, 5.14)} & \val{0.35}{0.19} & \val{0.22}{0.14} \\
	&& ILS-CSL\textsubscript{FCI} (t=1) &  \val{12.8}{3.54} & \val{(40.7, 40.7)}{(8.25, 8.25)} & \val{0.38}{0.24} & \val{0.22}{0.18} \\
	& & Ours (t=0) & \val{1.3}{1.0} & \val{(0, 0)}{(0, 0)} & \val{0.90}{0.07}& \val{1}{0} \\
	&& Ours (t=0.5) &&&& \\
	&& Ours (t=1) & \val{2.1}{1.22} & \val{(2, 2)}{(3.07, 3.07)}& \val{0.87}{0.06} & \val{0.95}[{0.07}  \\
	\bottomrule
\end{tabular}

==> tables/tbl_causal_discovery_metrics_t05_1.tex <==
\begin{tabular}{cclccccc}
	\toprule
	\textbf{Dataset} & \textbf{Approach} & \textbf{Method} & \textbf{Mod. SHD $\downarrow$} & \textbf{SID $\downarrow$} & \textbf{Precision $\uparrow$} & \textbf{Recall $\uparrow$} & \textbf{F1 Score $\uparrow$} \\
	\midrule
\multirow{10}{*}{\rotatebox{90}{\dataset{Earthquake}{5}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{2.00}{0.00} & \val{(0.00, 5.00)}{(0.00, 0.00)} & \val{1.00}{0.00} & \val{0.50}{0.00} & \val{0.67}{0.00} \\
	&& FCI-Vanilla & \val{3.60}{0.80} & \val{(8.20, 9.20)}{(3.60, 1.60)} & \val{0.20}{0.40} & \val{0.05}{0.10} & \val{0.08}{0.16} \\
	&& FCI-Iterative & \val{5.00}{1.67} & \val{(12.20, 12.20)}{(4.66, 4.66)} & \val{0.30}{0.27} & \val{0.20}{0.19} & \val{0.24}{0.22} \\
	&& FCI-Heuristics & \val{3.60}{0.80} & \val{(8.20, 9.20)}{(3.60, 1.60)} & \val{0.20}{0.40} & \val{0.05}{0.10} & \val{0.08}{0.16} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0)}} & LLM-first & \val{6.00}{0.82} & \val{(15.00, 15.00)}{(0.82, 0.82)} & \val{0.11}{0.16} & \val{0.08}{0.12} & \val{0.09}{0.13} \\
	&& ILS-CSL & \val{2.00}{0.89} & \val{(5.00, 5.00)}{(0.89, 0.89)} & \val{0.93}{0.13} & \val{0.55}{0.19} & \val{0.67}{0.17} \\
	 & & 	\cellcolor{highlight} \ours &	\cellcolor{highlight} \val{1.00}{0.63} &	\cellcolor{highlight} \val{(2.20, 2.20)}{(1.60, 1.60)} & 	\cellcolor{highlight} \val{1.00}{0.00} & 	\cellcolor{highlight} \val{0.75}{0.16} & 	\cellcolor{highlight} \val{0.85}{0.11}  \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0.5)}} & LLM-first & \val{6.00}{0.82} & \val{(15.00, 15.00)}{(0.82, 0.82)} & \val{0.11}{0.16} & \val{0.08}{0.12} & \val{0.09}{0.13} \\
	&& ILS-CSL & \val{2.00}{0.89} & \val{(5.00, 5.00)}{(2.61, 2.61)} & \val{0.93}{0.13} & \val{0.55}{0.19} & \val{0.67}{0.17} \\
	\rowcolor{highlight}\cellcolor{white} &\cellcolor{white}& \ours & \val{1.00}{0.63} & \val{(2.20, 2.20)}{(1.60, 1.60)} & \val{1.00}{0.00} & \val{0.75}{0.16} & \val{0.85}{0.11}  \\
	%	
	\midrule
	%	
	\multirow{10}{*}{\rotatebox{90}{\dataset{Asia}{8}}}  & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{7.00}{0.00} & \val{(23.00, 49.00)}{(0.00, 0.00)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
	&& FCI-Vanilla & \val{7.80}{0.75} & \val{(30.00, 35.00)}{(5.90, 2.45)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
	&& FCI-Iterative & \val{8.00}{1.26} & \val{(33.00, 33.00)}{(7.46, 7.46)} & \val{0.45}{0.24} & \val{0.23}{0.15} & \val{0.29}{0.18} \\
	&& FCI-Heuristics & \val{7.80}{0.75} & \val{(30.00, 35.00)}{(5.90, 2.45)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0)}} & LLM-first &\val{7.33}{0.94} & \val{(27.67, 27.67)}{(2.49, 2.49)} & \val{0.58}{0.12} & \val{0.29}{0.06} & \val{0.39}{0.08} \\
	&& ILS-CSL & \val{5.20}{0.75} & \val{(21.80, 21.80)}{(1.94, 1.94)} & \val{0.90}{0.10} & \val{0.38}{0.08} & \val{0.53}{0.09}  \\
   && \cellcolor{highlight}  \ours & \cellcolor{highlight}\val{4.60}{1.02}  & \cellcolor{highlight}\val{(13.60, 13.60)}{(3.83, 3.83)}  & \cellcolor{highlight}\val{0.80}{0.12} & \cellcolor{highlight}\val{0.60}{0.12} & \cellcolor{highlight}\val{0.67}{0.08}  \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0.5)}} & LLM-first &\val{7.33}{0.94} & \val{(27.67, 27.67)}{(2.49, 2.49)} & \val{0.58}{0.12} & \val{0.29}{0.06} & \val{0.39}{0.08} \\
	&& ILS-CSL & \val{5.60}{1.36} & \val{(22.80, 22.80)}{(3.19, 3.19)} & \val{0.85}{0.15} & \val{0.35}{0.09} & \val{0.49}{0.12}  \\
	&& \cellcolor{highlight}  \ours & \cellcolor{highlight}\val{4.60}{1.02}  & \cellcolor{highlight}\val{(13.60, 13.60)}{(3.83, 3.83)}  & \cellcolor{highlight}\val{0.80}{0.12} & \cellcolor{highlight}\val{0.60}{0.12} & \cellcolor{highlight}\val{0.67}{0.08}  \\
	%
	\midrule
	%	
	\multirow{10}{*}{\rotatebox{90}{\tiny\dataset{User Level Data-I}{9}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{15.00}{2.77} & \val{(47.80, 47.80)}{(4.62, 4.62)} & \val{0.72}{0.18} & \val{0.37}{0.09} & \val{0.47}{0.09} \\
	&& FCI-Vanilla & \val{21.30}{3.50} & \val{(61.60, 61.60)}{(5.54, 5.54)} & \val{0.41}{0.18} & \val{0.22}{0.10} & \val{0.29}{0.13} \\
	&& FCI-Iterative & \val{\phantom{0}5.60}{1.20} & \val{(23.40, 23.40)}{(7.94, 7.94)} & \val{0.93}{0.04} & \val{0.77}{0.02} & \val{0.84}{0.03} \\
	&& FCI-Heuristics & \val{21.30}{3.50} & \val{(61.60, 61.60)}{(5.54, 5.54)} & \val{0.41}{0.18} & \val{0.22}{0.10} & \val{0.29}{0.13} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0)}} & LLM-first & \val{8.40}{1.20} & \val{(35.20, 35.20)}{(2.92, 2.92)} & \val{0.83}{0.05} & \val{0.69}{0.02} & \val{0.76}{0.03}  \\
	&& ILS-CSL & \val{8.50}{2.60} & \val{(30.25, 30.25)}{(9.09, 9.09)} & \val{0.83}{0.08} & \val{0.69}{0.08} & \val{0.75}{0.07}  \\
	&& \cellcolor{highlight}  \ours & \cellcolor{highlight}\val{5.40}{0.49}  & \cellcolor{highlight}\val{(13.20, 13.20)}{(2.40, 2.40)} & \cellcolor{highlight}\val{0.88}{0.02} & \cellcolor{highlight}\val{0.83}{0.02} & \cellcolor{highlight}\val{0.85}{0.01} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0.5)}} & LLM-first & \val{9.60}{1.69} & \val{(38.70, 38.70)}{(4.94, 4.94)} & \val{0.80}{0.06} & \val{0.67}{0.03} & \val{0.73}{0.05}  \\
	&& ILS-CSL & \val{7.67}{1.70} & \val{(26.33, 26.33)}{(3.68, 3.68)} & \val{0.84}{0.05} &\val{0.74}{0.04}& \val{0.79}{0.05}  \\
	&& \cellcolor{highlight}  \ours & \cellcolor{highlight}\val{4.60}{0.49}  & \cellcolor{highlight}\val{(12.00, 12.00)}{(0.00, 0.00)} & \cellcolor{highlight}\val{0.91}{0.03} & \cellcolor{highlight}\val{0.84}{0.00} & \cellcolor{highlight}\val{0.87}{0.01}  \\
	%	
	\midrule
	%	
	\multirow{10}{*}{\rotatebox{90}{\tiny\dataset{User Level Data-II}{8}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{19.80}{2.04} & \val{(40.00, 40.00)}{(3.03, 3.03)} & \val{0.15}{0.07} & \val{0.10}{0.04} & \val{0.12}{0.05} \\
	&& FCI-Vanilla & \val{17.40}{1.83} & \val{(36.80, 39.40)}{(2.04, 3.38)} & \val{0.07}{0.13} & \val{0.02}{0.03} & \val{0.03}{0.05} \\
	&& FCI-Iterative & \val{20.60}{1.77} & \val{(42.80, 43.40)}{(4.07, 4.22)} & \val{0.06}{0.08} & \val{0.05}{0.07} & \val{0.05}{0.07} \\
	&& FCI-Heuristics & \val{17.40}{1.83} & \val{(36.80, 39.40)}{(2.04, 3.38)} & \val{0.07}{0.13} & \val{0.02}{0.03} & \val{0.03}{0.05} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0)}} & LLM-first & \val{18.33}{0.94}&\val{(42.67, 42.67)}{(0.47, 0.47)}&\val{0.21}{0.04}&\val{0.19}{0.04}&\val{0.20}{0.04} \\
	&& ILS-CSL &\val{19.00}{1.22}&\val{(46.75, 46.75)}{(4.87, 4.87)}&\val{0.14}{0.06}&\val{0.13}{0.07}&\val{0.13}{0.07} \\
	&& \cellcolor{highlight}  \ours & \cellcolor{highlight}\val{18.67}{1.70}  & \cellcolor{highlight}\val{(41.00, 41.00)}{(1.63,1.63)} & \cellcolor{highlight}\val{0.22}{0.02} & \cellcolor{highlight}\val{0.22}{0.04} & \cellcolor{highlight}\val{0.22}{0.02} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0.5)}} & LLM-first &\val{18.33}{0.94}&\val{(42.67, 42.67)}{(0.47, 0.47)}&\val{0.21}{0.04}&\val{0.19}{0.04}&\val{0.20}{0.04} \\
	&& ILS-CSL &\val{17.60}{2.33}&\val{(41.20, 41.20)}{(4.12, 4.12)}&\val{0.21}{0.11}&\val{0.18}{0.12}&\val{0.19}{0.12}\\
	&& \cellcolor{highlight}  \ours & \cellcolor{highlight}\val{18.67}{2.05}  & \cellcolor{highlight}\val{(41.00, 41.00)}{(1.63,1.63)} & \cellcolor{highlight}\val{0.23}{0.02} & \cellcolor{highlight}\val{0.22}{0.04} & \cellcolor{highlight}\val{0.22}{0.02}  \\
	%	
	\midrule
	%	
	\multirow{10}{*}{\rotatebox{90}{\dataset{Child}{19}}}  & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{27.50}{0.00} & \val{(111.00, 131.00)}{(\phantom{0}0.00, \phantom{0}0.00)} & \val{0.38}{0.00} & \val{0.36}{0.00} & \val{0.37}{0.00} \\
	&& FCI-Vanilla & \val{28.00}{1.48} & \val{(129.20, 133.20)}{(10.46, 10.76)} & \val{0.38}{0.04} & \val{0.26}{0.05} & \val{0.31}{0.04} \\
	&& FCI-Iterative & \val{32.10}{1.16} & \val{(149.00, 164.40)}{(\phantom{0}7.16, 10.33)} & \val{0.27}{0.03} & \val{0.26}{0.04} & \val{0.26}{0.03} \\
	&& FCI-Heuristics & \val{28.00}{1.48} & \val{(129.20, 133.20)}{(10.46, 10.76)} & \val{0.38}{0.04} & \val{0.26}{0.05} & \val{0.31}{0.04} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0)}} & LLM-first & \val{29.67}{0.47} & \val{(154.83, 154.83)}{(\phantom{0}9.75, \phantom{0}9.75)} & \val{0.33}{0.01} & \val{0.35}{0.02} & \val{0.34}{0.01} \\
	&& ILS-CSL & \val{29.80}{2.48} & \val{(160.00, 160.00)}{(21.25, 21.25)} & \val{0.33}{0.05} & \val{0.35}{0.04} & \val{0.34}{0.04}  \\
	 & &  \cellcolor{highlight} \ours &  \cellcolor{highlight}\val{27.80}{0.75} &  \cellcolor{highlight} \val{(114.80, 114.80)}{(\phantom{0}7.76, \phantom{0}7.76)} &  \cellcolor{highlight} \val{0.39}{0.01} &  \cellcolor{highlight} \val{0.45}{0.03} &  \cellcolor{highlight} \val{0.42}{0.02} \\
	\cdashline{2-8}[.4pt/1pt]
		& \multirow{3}{*}{Data-LM\textsubscript{(t=0.5)}} & LLM-first & \val{30.67}{1.11} & \val{(146.83, 146.83)}{(\phantom{0}4.81, \phantom{0}4.81)} & \val{0.31}{0.03} & \val{0.32}{0.03} & \val{0.32}{0.03} \\
	&& ILS-CSL & \val{32.00}{2.28} & \val{(152.80, 152.80)}{(12.95, 12.95)} & \val{0.28}{0.05} & \val{0.29}{0.06} & \val{0.28}{0.06}  \\
	\rowcolor{highlight}\cellcolor{white} &\cellcolor{white}& \ours & \val{28.10}{0.86} & \val{(100.60, 112.00)}{(\phantom{0}9.31, \phantom{0}0.00)} & \val{0.40}{0.01} & \val{0.45}{0.00} & \val{0.42}{0.01} \\
	%	
	\midrule
	%	
	\multirow{10}{*}{\rotatebox{90}{\dataset{Alarm}{37}}} & \multirow{4}{*}{Only-Data} & FCI-Cumulative & \val{45.00}{0.00} & \val{(626.00, 626.00)}{(\phantom{0}0.00, \phantom{0}0.00)} & \val{0.25}{0.00} & \val{0.02}{0.00} & \val{0.04}{0.00} \\
	&& FCI-Vanilla & \val{49.50}{1.61} & \val{(617.80, 699.20)}{(29.23, 68.43)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
	&& FCI-Iterative & \val{52.40}{6.21} & \val{(612.20, 636.80)}{(49.87, 43.83)} & \val{0.33}{0.14} & \val{0.12}{0.05} & \val{0.17}{0.07} \\
	&& FCI-Heuristics & \val{49.50}{1.61} & \val{(617.80, 699.20)}{(29.23, 68.43)} & \val{0.00}{0.00} & \val{0.00}{0.00} & \val{0.00}{0.00} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0)}} & LLM-first & \val{57.33}{1.89} & \val{(695.33, 695.33)}{(21.91, 21.91)} & \val{0.22}{0.03} & \val{0.10}{0.01} & \val{0.13}{0.01} \\
	&& ILS-CSL & \val{49.50}{1.50} & \val{(647.50, 647.50)}{(18.94, 18.94)} & \val{0.39}{0.05} & \val{0.10}{0.02} & \val{0.17}{0.03} \\
	 & & \cellcolor{highlight} \ours & \cellcolor{highlight} \val{51.60}{1.77} & \cellcolor{highlight} \val{(595.00, 595.80)}{(16.63, 16.94)} & \cellcolor{highlight} \val{0.40}{0.04} & \cellcolor{highlight} \val{0.22}{0.01} & \cellcolor{highlight} \val{0.28}{0.01} \\
	\cdashline{2-8}[.4pt/1pt]
	& \multirow{3}{*}{Data-LM\textsubscript{(t=0.5)}} & LLM-first & \val{56.67}{2.49} & \val{(684.67, 684.67)}{(16.34, 16.34)} & \val{0.23}{0.05} & \val{0.10}{0.02} & \val{0.14}{0.03} \\
   && ILS-CSL & \val{49.75}{1.48} & \val{(633.25, 633.25)}{(13.05, 13.05)} & \val{0.41}{0.02} & \val{0.12}{0.01} & \val{0.19}{0.01}  \\
	& & \cellcolor{highlight} \ours & \cellcolor{highlight} \val{51.70}{1.29} & \cellcolor{highlight} \val{(594.00, 595.20)}{(38.75, 38.75)} & \cellcolor{highlight} \val{0.41}{0.03} & \cellcolor{highlight} \val{0.22}{0.02} & \cellcolor{highlight} \val{0.29}{0.02} \\
	\bottomrule
\end{tabular}



==> tables/tbl_fci_pairwise.tex <==
\begin{tabular}{cccccc}
	\toprule
	\textbf{Dataset} & \textbf{Temp.} & \textbf{Method} & \textbf{SHD} & \textbf{Precision} & \textbf{Recall} \\
	\midrule
	\multirow{6}{*}{Earthquake} 
	& \multirow{2}{*}{0}  & Pairwise & \val{3.0}{0.00} & \val{0.57}{0.00} & \val{1.00}{0.00} \\
	&     & FCI-Pairwise  & \val{1.6}{0.91} & \val{0.91}{0.14} & \val{0.68}{0.16} \\
	& \multirow{2}{*}{0.5} & Pairwise & \val{2.4}{0.66} & \val{0.63}{0.07} & \val{1.00}{0.00} \\
	&     & FCI-Pairwise  & \val{2.9}{0.60} & \val{0.84}{0.16}&\val{0.58}{0.11} \\
	& \multirow{2}{*}{1} & Pairwise & \val{2.2}{0.75} & \val{0.65}{0.07} & \val{0.98}{0.07} \\
	&     & FCI-Pairwise  & \val{2.8}{1.25} & \val{0.76}{0.20}& \val{0.68}{0.16} \\
	\midrule
	\multirow{6}{*}{Asia} 
	& \multirow{2}{*}{0}  & Pairwise & \val{22.0}{0.77} & \val{0.27}{0.01}  &\val{1.00}{0.00}\\
	&     & FCI-Pairwise  & \val{17.65}{0.84} & \val{0.25}{0.02} & \val{0.48}{0.05} \\
	& \multirow{2}{*}{0.5} & Pairwise & \val{22.2}{1.66} & \val{0.26}{0.02}  & \val{0.98}{0.05} \\
	&     & FCI-Pairwise  & \val{18.25}{1.19} & \val{0.27}{0.03} & \val{0.55}{0.83} \\
	& \multirow{2}{*}{1}   & Pairwise & \val{20.6}{1.85} & \val{0.28}{0.02}  & \val{0.96}{0.06} \\
	&     & FCI-Pairwise & \val{21.4}{2.09} & \val{0.26}{0.06} & \val{0.43}{0.13} \\
	\midrule
	\multirow{6}{*}{Google User} 
	& \multirow{2}{*}{0}  & Pairwise & \val{49.9}{0.83} & \val{(59.3, 59.3)}{(3.52, 3.52)}  & \\
	&     & FCI-Pairwise & \val{39.1}{0.97} & \val{(54.2, 54.2)}{(4.10, 4.10)} & \\
	& \multirow{2}{*}{0.5} & Pairwise & \val{50.7}{1.42} & \val{(61.1, 61.1)}{(2.21, 2.21)}  & \\
	&     & FCI-Pairwise & \val{38.8}{2.55} & \val{(52.0, 52.0)}{(5.08, 5.08)} & \\
	& \multirow{2}{*}{1}   & Pairwise & \val{49.4}{1.28} & \val{(59.7, 59.7)}{(3.49, 3.49)}  & \\
	&     & FCI-Pairwise & \val{37.6}{2.21} & \val{(50.1, 50.1)}{(4.99, 4.99)} & \\
	\bottomrule
\end{tabular}
 

==> tables/tbl_llm_overly_optimistic.tex <==
\begin{tabular}{ccl ccc ccc}
	\toprule
	\textbf{Dataset} & \textbf{Temp.} & \textbf{Method} & \multicolumn{3}{c}{\textbf{GPT-3.5\textsubscript{turbo}}} &\multicolumn{3}{c}{\textbf{GPT-4o}}  \\
	\midrule
	&&&\textbf{SHD} $\downarrow$ & \textbf{Precision} $\uparrow$ & \textbf{Recall} $\uparrow$ & \textbf{SHD} $\downarrow$ & \textbf{Precision} $\uparrow$ & \textbf{Recall} $\uparrow$ \\
	\midrule
	\multirow{6}{*}{\rotatebox{90}{\sc Earthquake}} 
	& \multirow{2}{*}{0.0}   & Pairwise & \val{3.0}{0.0} & \val{0.57}{0.00} & \val{1.0}{0.0} & \val{2.0}{0.0} & \val{0.67}{0.00} & \val{1.0}{0.0} \\
	&     & Triplet  & \val{2.1}{0.3}  & \val{0.66}{0.03} & \val{1.0}{0.0}  & \val{4.8}{0.4} & \val{0.46}{0.02} & \val{1.0}{0.0}  \\
	\cdashline{2-9}[.4pt/2pt]
	& \multirow{2}{*}{0.5} & Pairwise & \val{2.8}{0.6} & \val{0.59}{0.05} & \val{1.0}{0.0}  & \val{2.2}{0.4} & \val{0.65}{0.04} & \val{1.0}{0.0} \\
	&     & Triplet  & \val{2.1}{0.3}  & \val{0.66}{0.03} & \val{1.0}{0.0}  & \val{4.4}{0.5} & \val{0.48}{0.03} & \val{1.0}{0.0} \\
		\cdashline{2-9}[.4pt/2pt]
	& \multirow{2}{*}{1.0}  & Pairwise & \val{3.2}{0.6} & \val{0.56}{0.05} & \val{1.0}{0.0}  & \val{1.8}{0.4} & \val{0.69}{0.05} & \val{1.0}{0.0} \\
	&     & Triplet  & \val{2.0}{0.6}   & \val{0.67}{0.07} & \val{1.0}{0.0}  & \val{6.2}{0.8} & \val{0.39}{0.03} & \val{1.0}{0.0} \\
	\midrule
	\multirow{6}{*}{\rotatebox{90}{\sc Asia}} 
	& \multirow{2}{*}{0.0}   & Pairwise & \val{25.2}{0.4}   & \val{0.24}{0.00} & \val{1.0}{0.0}  &\val{11.2}{0.4}& \val{0.42}{0.01} & \val{1.0}{0.0} \\
	&     & Triplet  & \val{24.5}{0.5}  & \val{0.25}{0.00} & \val{1.0}{0.0}  & \val{19.0}{0.6} & \val{0.30}{0.01} & \val{1.0}{0.0} \\
			\cdashline{2-9}[.4pt/2pt]
	& \multirow{2}{*}{0.5} & Pairwise & \val{23.4}{1.0}  & \val{0.26}{0.01} & \val{1.0}{0.0}  & \val{11.6}{0.5} & \val{0.48}{0.01} & \val{1.0}{0.0} \\
	&     & Triplet  & \val{24.0}{1.0}      & \val{0.25}{0.01} & \val{1.0}{0.0}  & \val{19.2}{0.8} &\val{0.29}{0.01}&\val{1.0}{0.0} \\
			\cdashline{2-9}[.4pt/2pt]
	& \multirow{2}{*}{1.0}   & Pairwise & \val{23.2}{1.5} & \val{0.25}{0.02} & \val{0.9}{0.1}  & \val{11.8}{0.4} & \val{0.40}{0.01} & \val{1.0}{0.0}  \\
	&     & Triplet  & \val{23.3}{1.0} & \val{0.26}{0.01} & \val{1.0}{0.0}  &\val{26.2}{1.7}&\val{0.23}{0.01}&\val{1.0}{0.0}  \\
	\bottomrule
\end{tabular}


==> tables/tbl_notations.tex <==
\begin{tabular}{@{}ll ll ll@{}}
	\toprule
	\textbf{Symbol} & \textbf{Description} &
	\textbf{Symbol} & \textbf{Description} &
	\textbf{Symbol} & \textbf{Description} \\
	\midrule
	\multicolumn{6}{@{}l}{\textbf{Dataset and Observations}} \\
	$ \mathbb{D}$ & True data distribution & 
	$\mathcal{D}$ & Full observed dataset & 
	$\DD_i$ & Observed data at batch $i$ \\
	$n_i$ & Number of data points in batch $i$ & 
	$\VD$ & Set of observed variables & 
	$d$ & Cardinality of $\VD$ \\
	$\VL$ & Unobserved (latent) variables & 
	$k$ & Look-back batch window size & 
	$\B_i$ & Background knowledge till batch $i$ \\
	\midrule
	\multicolumn{6}{@{}l}{\textbf{Causal Graphs and Structures}} \\
	$\G$ & True underlying causal graph & 
	$\V, \E$ & Nodes and edges in $\G$ & 
	$\GD{i}$ & Causal graph after batch $i$ \\
	$\VD, \ED{i}$ & Nodes/edges in $\GD{i}$ & 
	$\GE{i}$ & Expert-provided graph till batch {i} & 
	$\VE{i}, \EE{i}$ & Nodes and edges in $\GE{i}$ \\
	$A, B$ & Arbitrary variables in graph & 
	$L$ & Latent confounder in causal structure& 
	&  \\
	\midrule
	\multicolumn{6}{@{}l}{\textbf{Parameters and Models}} \\
	$\vtheta$ & Edge weights of the causal DAG & 
	$\vthetaO, \vthetaL$ & Edge weights for observed, latent variable & 
	$\vphi$ & SEM parameters $\{\vtheta, \sigma^2\}$ \\
	$\theta_{A}$ & Edge weights associated with $A$ & 
	$\vphi_{A}$ & Parameters for $A$ variable ($\theta_A, \sigma^2$) & 
	$\epsilon$ & SEM noise \\
	$\sigma^2$ & SEM noise variance & 
	$\rho(A, B)$ & Correlation value between $A, B$ & 
	& \\
	\midrule
	\multicolumn{6}{@{}l}{\textbf{Expert Interaction and Histograms}} \\
	$\alpha$ & Expert noise level & 
	$\HE{i}$ & Edge histogram till batch $i$ & 
	$\HL{i}$ & Latent variable histogram till batch $i$ \\
	$\IE, \IL$ & Instructions for edge/latent expert & 
	$\IP, \IR$ & Instructions for prior/correlation expert. & 
	$\me, \ml$ & Maximum expert calls for edge/latent \\
	\midrule
	\multicolumn{6}{@{}l}{\textbf{Others}} \\
	$\R$ & Set of real numbers & 
	$\N$ & Gaussian distribution & 
	$\eta$ & Learning rate \\
	$\lambda$ & Regularizer parameter & 
	$\vm_p$ & Prior mean & 
	$\MS_p$ & Prior covariance \\
	\bottomrule
\end{tabular}


==> tables/tbl_pag_llm.tex <==
\begin{tabular}{cclc}
	\toprule
	\textbf{Dataset} & \textbf{Temp.} & \textbf{Method} & \textbf{SID} $\downarrow$ \\
	\midrule
	\multirow{6}{*}{\rotatebox{90}{\sc Earthquake}} 
	& \multirow{2}{*}{0.0}   & Pairwise (Voting) & \val{(1.0, 1.0)}{(0.0, 0.0)}   \\
	 & & \cellcolor{highlight}{PAG-Pairwise}  &\cellcolor{highlight}{\val{(0.0, 0.0)}{(0.0, 0.0)}} \\
	\cdashline{2-4}[.4pt/2pt]
	& \multirow{2}{*}{0.5} & Pairwise (Voting)  & \val{(1.4, 1.4)}{(1.2, 1.2)}  \\
	 & & \cellcolor{highlight}{PAG-Pairwise}   & \cellcolor{highlight}{\val{(0.0, 0.0)}{(0.0, 0.0)}} \\
	\cdashline{2-4}[.4pt/2pt]
	& \multirow{2}{*}{1.0} & Pairwise (Voting)  & \val{(1.6, 1.6)}{(1.5, 1.5)} \\
	 &  & \cellcolor{highlight}{PAG-Pairwise}  & \cellcolor{highlight}{\val{(0.8, 0.8)}{(1.6, 1.6)}} \\
	\midrule
	\multirow{6}{*}{\rotatebox{90}{\sc Asia}} 
	& \multirow{2}{*}{0.0}   & Pairwise (Voting) &\val{(6.4, 6.4)}{(0.8, 0.8)} \\
	& & \cellcolor{highlight}{PAG-Pairwise}  & \cellcolor{highlight}{\val{(3.8, 3.8)}{(0.9, 0.9)}} \\
	\cdashline{2-4}[.4pt/2pt]
	& \multirow{2}{*}{0.5} & Pairwise (Voting) &\val{(5.2, 5.2)}{(1.7, 1.7)} \\
	 & & \cellcolor{highlight}{PAG-Pairwise} & \cellcolor{highlight}{\val{(3.5, 3.5)}{(0.8, 0.8)}} \\
	\cdashline{2-4}[.4pt/2pt]
	& \multirow{2}{*}{1.0}   & Pairwise (Voting) &\val{(5.4, 5.4)}{(1.8, 1.8)} \\
	&  & \cellcolor{highlight}{PAG-Pairwise} & \cellcolor{highlight}{\val{(4.0, 4.0)}{(1.9, 1.9)}}  \\
	\bottomrule
\end{tabular}


==> tables/tbl_qwen_llama.tex <==
\begin{tabular}{cllccccc}
	\toprule
	\textbf{Dataset} & \textbf{Model} & \textbf{Method} & \textbf{Mod. SHD $\downarrow$} & \textbf{SID $\downarrow$} & \textbf{Precision $\uparrow$} & \textbf{Recall $\uparrow$} & \textbf{F1 Score $\uparrow$}\\
	\midrule
	\multirow{11}{*}{\rotatebox{90}{\tiny{ \sc Child}}} & \multirow{3}{*}{Llama3.1\textsubscript{8B-instruct}} & LLM-first 
	    & \val{45.80}{1.94} 
	    & \val{(211.20,\,211.20)}{(15.25,\,15.25)} 
	    & \val{0.13}{0.01} 
	    & \val{0.19}{0.02}
        & \val{0.16}{0.01}\\
    && ILS-CSL 
        & \val{27.60}{2.24} 
        & \val{(146.40,\,146.40)}{(15.93,\,15.93)} 
        & \val{0.37}{0.05} 
        & \val{0.38}{0.07}
        & \val{0.38}{0.06}\\
    % && BFS
    %     & --
    %     & --
    %     & --
    %     & --
    %     & -- \\
    & &\cellcolor{highlight} \ours 
	    &\cellcolor{highlight} \valb{24.60}{0.80} 
	    &\cellcolor{highlight} \valb{(101.80,\,101.80)}{(8.11,\,8.11)} 
	    &\cellcolor{highlight} \valb{0.44}{0.01} 
	    &\cellcolor{highlight} \valb{0.45}{0.02}
        &\cellcolor{highlight} \valb{0.44}{0.01}\\
    \cdashline{2-8}[.4pt/1pt]
    &\multirow{3}{*}{Qwen3\textsubscript{4B-instruct}} & LLM-first 
	    & \val{35.80}{2.04} 
	    & \val{(173.80,\,173.80)}{(14.13,\,14.13)} 
	    & \val{0.27}{0.02} 
	    & \valb{0.42}{0.02}
        & \val{0.34}{0.01} \\
    && ILS-CSL 
        & \val{30.60}{2.42} 
        & \val{(196.80,\,196.80)}{(14.13,\,14.13)} 
        & \val{0.30}{0.06} 
        & \val{0.28}{0.05}
        & \val{0.29}{0.05}\\
    % && BFS
    %     & --
    %     & --
    %     & --
    %     & --
    %     & -- \\
    && \cellcolor{highlight} \ours 
	    & \cellcolor{highlight} \valb{21.20}{0.75} 
	    & \cellcolor{highlight} \valb{(107.80,\,107.80)}{(13.42,\,13.42)} 
	    & \cellcolor{highlight} \valb{0.51}{0.01} 
	    & \cellcolor{highlight} \val{0.32}{0.03}
        & \cellcolor{highlight} \valb{0.39}{0.02}\\
    \cdashline{2-8}[.4pt/1pt]
    &\multirow{5}{*}{GPT4.1\textsubscript{nano}} & LLM-first 
	    & \val{31.83}{2.61}
        & \val{(203.50, 203.50)}{(23.06, 23.06)}
        & \val{0.16}{0.01}
        & \val{0.14}{0.03}
        & \val{0.15}{0.02} \\
    && ILS-CSL 
        & \val{31.60}{2.06}
        & \valb{(147.40, 147.40)}{(11.25, 11.25)}
        & \val{0.29}{0.05}
        & \val{0.19}{0.04}
        & \val{0.23}{0.03} \\
    && BFS 
        & \val{34.75}{7.80}
        & \val{(252.50, 252.50)}{(23.36, 23.36)}
        & \val{0.18}{0.08}
        & \val{0.12}{0.04}
        & \val{0.14}{0.03}  \\
    && BFS\textsubscript{corr} 
        & \val{32.30}{4.16}
        & \val{(301.10, 301.10}{(14.42, 14.42)}
        & \val{0.21}{0.03}
        & \val{0.15}{0.01}
        & \val{0.18}{0.01} \\
    && \cellcolor{highlight} \ours 
	    & \valb{27.90}{1.61} \cellcolor{highlight}
	    & \valb{(143.50, 165.50)}{(12.23, 35.97)} \cellcolor{highlight}
	    & \valb{0.42}{0.06} \cellcolor{highlight}
	    & \valb{0.23}{0.04} \cellcolor{highlight}
        & \valb{0.30}{0.03} \cellcolor{highlight}\\
	\midrule
	\multirow{11}{*}{\rotatebox{90}{\tiny{ \sc User Level Data-I}}} & \multirow{3}{*}{Llama3.1\textsubscript{8B-instruct}} & LLM-first 
	    & \val{11.50}{0.50} 
	    & \val{(42.50,\,42.50)}{(1.50,\,1.50)} 
	    & \val{0.74}{0.01} 
	    & \val{0.61}{0.03}
        & \val{0.67}{0.02} \\
    && ILS-CSL 
        & \val{9.75}{1.64} 
        & \val{(32.25,\,32.25)}{(3.56,\,3.56)} 
        & \val{0.78}{0.05} 
        & \val{0.66}{0.03}
        & \val{0.72}{0.04}\\
    && \cellcolor{highlight}\ours 
	    & \cellcolor{highlight}\valb{7.50}{0.45} 
	    & \cellcolor{highlight}\valb{(25.80,\,25.40)}{(2.32,\,4.22)} 
	    & \cellcolor{highlight}\valb{0.92}{0.07} 
	    & \cellcolor{highlight}\valb{0.69}{0.01}
        & \cellcolor{highlight}\valb{0.79}{0.01} \\
    \cdashline{2-8}[.4pt/1pt]
    &\multirow{3}{*}{Qwen3\textsubscript{4B-instruct}} & LLM-first 
	    & \val{23.67}{1.11} 
	    & \val{(64.33,\,64.33)}{(0.94,\,0.94)} 
	    & \val{0.35}{0.04} 
	    & \val{0.28}{0.04}
        & \val{0.31}{0.04}\\
    && ILS-CSL 
        & \val{20.60}{4.18} 
        & \val{(56.80,\,56.80)}{(7.36,\,7.36)} 
        & \val{0.45}{0.13} 
        & \val{0.36}{0.10}
        & \val{0.40}{0.12}\\
    & & \cellcolor{highlight} \ours 
	    & \cellcolor{highlight} \valb{9.80}{2.04} 
	    & \cellcolor{highlight} \valb{(26.60,\,26.60)}{(6.83,\,6.83)} 
	    & \cellcolor{highlight} \valb{0.91}{0.08} 
	    & \cellcolor{highlight} \valb{0.54}{0.08}
        & \cellcolor{highlight} \valb{0.67}{0.07}\\
    \cdashline{2-8}[.4pt/1pt]
    &\multirow{5}{*}{GPT4.1\textsubscript{nano}} & LLM-first 
	    & \val{19.42}{1.14}
	    & \val{(72.10, 72.10)}{(5.36, 5.36)}
	    & \val{0.76}{0.07}
	    & \val{0.32}{0.03}
	    & \val{0.45}{0.03} \\
    && ILS-CSL 
        & \val{18.00}{1.41}
        & \val{(54.00, 54.00)}{(2.53, 2.53)}
        & \val{0.53}{0.05}
        & \valb{0.42}{0.03}
        & \val{0.47}{0.04} \\
    && BFS 
        & \val{36.60}{8.96}
        & \val{(65.80, 65.80)}{(2.17, 2.17)}
        & \val{0.13}{0.06}
        & \val{0.29}{0.14}
        & \val{0.18}{0.06}\\
    && BFS\textsubscript{corr} 
        & \val{24.00}{6.24}
        & \val{(42.20, 42.20)}{(6.53, 6.53)}
        & \val{0.17}{0.12}
        & \val{0.28}{0.11}
        & \val{0.21}{0.11}\\
    && \cellcolor{highlight} \ours 
	    & \valb{10.60}{2.13} \cellcolor{highlight}
	    & \valb{(34.80, 35.20)}{(5.56, 5.84)} \cellcolor{highlight}
	    & \valb{0.97}{0.04} \cellcolor{highlight}
	    & \valb{0.43}{0.06} \cellcolor{highlight}
        & \valb{0.60}{0.06} \cellcolor{highlight}\\
	\bottomrule
\end{tabular}

==> tables/tbl_sid_noise_levels.tex <==
\begin{tabular}{|c|*{7}{c|c|}}
	\hline
	{} & \multicolumn{2}{c|}{Batch 1} & \multicolumn{2}{c|}{Batch 2} & \multicolumn{2}{c|}{Batch 3} & \multicolumn{2}{c|}{Batch 4} & \multicolumn{2}{c|}{Batch 5} & \multicolumn{2}{c|}{Batch 6} & \multicolumn{2}{c|}{Batch 7} \\
	\hline
	{$\rho$} & LB & UB & LB & UB & LB & UB & LB & UB & LB & UB & LB & UB & LB & UB \\
	\hline
	\multicolumn{15}{|c|}{Score Selection} \\
	\hline
	$0.1$ & \val{36.2}{3.7} & \val{36.2}{3.7} & \val{11.6}{1.2} & \val{11.6}{1.2} & \val{11.6}{1.2} & \val{11.6}{1.2} & \val{10.8}{1.8} & \val{10.8}{1.8} & \val{10.1}{2.5} & \val{10.1}{2.5} & \val{9.7}{3.4} & \val{9.7}{3.4} & \val{9.3}{3.4} & \val{9.3}{3.4} \\
	$0.3$ & \val{46.3}{3.3} & \val{46.3}{3.3} & \val{13.8}{4.5} & \val{13.8}{4.5} & \val{9.4}{2.5} & \val{9.4}{2.5} & \val{8.9}{2.2} & \val{8.9}{2.2} & \val{8.5}{3.1} & \val{8.5}{3.1} & \val{7.8}{3.0} & \val{7.8}{3.0} & \val{7.8}{3.0} & \val{7.8}{3.0} \\
	$0.5$ & \val{49.5}{2.3} & \val{49.5}{2.3} & \val{40.0}{4.5} & \val{40.0}{4.5} & \val{28.1}{5.1} & \val{28.1}{5.1} & \val{25.8}{4.5} & \val{25.8}{4.5} & \val{21.6}{5.9} & \val{21.6}{5.9} & \val{18.8}{5.2} & \val{18.8}{5.2} & \val{15.9}{5.4} & \val{15.9}{5.4} \\
	$0.7$ & \val{50.9}{0.3} & \val{50.9}{0.3} & \val{50.5}{0.7} & \val{50.5}{0.7} & \val{49.9}{1.1} & \val{49.9}{1.1} & \val{49.6}{1.1} & \val{49.6}{1.1} & \val{49.6}{1.1} & \val{49.6}{1.1} & \val{49.6}{1.1} & \val{49.6}{1.1} & \val{48.9}{1.9} & \val{48.9}{1.9} \\
	$0.9$ & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} \\
	\hline
	\multicolumn{15}{|c|}{Random Selection} \\
	\hline
	$0.1$ & \val{43.2}{4.5} & \val{43.2}{4.5} & \val{13.9}{3.2} & \val{13.9}{3.2} & \val{11.4}{2.7} & \val{11.4}{2.7} & \val{9.8}{2.6} & \val{9.8}{2.6} & \val{9.8}{2.6} & \val{9.8}{2.6} & \val{9.8}{2.6} & \val{9.8}{2.6} & \val{9.4}{2.5} & \val{9.4}{2.5} \\
	$0.3$ & \val{47.7}{3.3} & \val{47.7}{3.3} & \val{23.0}{5.4} & \val{23.0}{5.4} & \val{12.7}{3.0} & \val{12.7}{3.0} & \val{10.9}{2.8} & \val{10.9}{2.8} & \val{9.6}{2.0} & \val{9.6}{2.0} & \val{9.6}{2.0} & \val{9.6}{2.0} & \val{9.6}{2.0} & \val{9.6}{2.0} \\
	$0.5$ & \val{50.7}{0.5} & \val{50.7}{0.5} & \val{41.7}{3.0} & \val{41.7}{3.0} & \val{37.6}{5.6} & \val{37.6}{5.6} & \val{35.2}{5.9} & \val{35.2}{5.9} & \val{33.2}{6.2} & \val{33.2}{6.2} & \val{32.1}{6.5} & \val{32.1}{6.5} & \val{30.4}{6.2} & \val{30.4}{6.2} \\
	$0.7$ & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} & \val{50.8}{0.4} \\
	$0.9$ & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} & \val{51.0}{0.0} \\
	\hline
\end{tabular}

